A Safe Harbor for AI Evaluation and Red Teaming

Independent evaluation and red teaming are critical for identifying the risks posed by generative AI systems. However, the terms of service and enforcement strategies used by prominent AI companies to deter model misuse have disincentives on good faith safety evaluations. This causes some researchers to fear that conducting such research or releasing their findings will result in account suspensions or legal reprisal. Although some companies offer researcher access programs, they are an inadequate substitute for independent research access, as they have limited community representation, receive inadequate funding, and lack independence from corporate incentives. We propose that major AI developers commit to providing a legal and technical safe harbor, indemnifying public interest safety research and protecting it from the threat of account suspensions or legal reprisal. These proposals emerged from our collective experience conducting safety, privacy, and trustworthiness research on generative AI systems, where norms and incentives could be better aligned with public interests, without exacerbating model misuse. We believe these commitments are a necessary step towards more inclusive and unimpeded community efforts to tackle the risks of generative AI.

==> acknowledgements.tex <==
\paragraph{Acknowledgements.}
We thank \todo{}

\paragraph{Funding.}

\paragraph{Conflicts of Interest.}


==> tables/policies-hyperlinks.tex <==
\begin{table*}[t!]
\centering
\footnotesize
\renewcommand{\arraystretch}{1.5}
\begin{adjustbox}{width=\textwidth}
\begin{tabular}{p{3.5cm} | p{2.4cm}p{2.4cm}p{2.4cm}p{2.4cm}p{2.4cm}p{2.4cm}}
\toprule
 & \textsc{OpenAI} & \textsc{Google} & \textsc{Anthropic} & \textsc{Inflection} & \textsc{Meta} & \textsc{Midjourney} \\
\midrule
\textbf{AI System} & GPT-4 & Gemini & Claude 2 & Inflection-1 & Llama 2 & Midjourney v6 \\
\textbf{Public API} & \href{http://chat.openai.com}{Y} & \href{https://ai.google.dev/}{Y} & \href{https://support.anthropic.com/en/articles/8114521-how-can-i-access-the-claude-api}{N} & N & N & N \\
% \textbf{Deep Access} & Top-5 logits & N & N & N & Open weights & N \\
\textbf{Researcher Access} & \href{https://openai.com/form/researcher-access-program}{Y} & N & Y \href{https://www.anthropic.com/earlyaccess} & N & \href{https://ai.meta.com/resources/models-and-libraries/llama-downloads/}{Open weights}  & N \\
\textbf{Bug Bounty} & \href{https://bugcrowd.com/openai}{Y} & \href{https://security.googleblog.com/2023/10/googles-reward-criteria-for-reporting.html}{Y} & N & N & \href{https://www.facebook.com/whitehat/info/}{Y} & N \\
\textbf{Safe Harbor} & \href{https://bugcrowd.com/openai}{Security \& Academic Safety} & N & \href{https://www.anthropic.com/responsible-disclosure-policy}{Security only*} & N & \href{https://www.facebook.com/whitehat/info/}{Security only*} & N \\
\midrule
\multicolumn{7}{c}{\textsc{\emph{Enforcement Policy Disclosures}}} \\
\midrule
\textbf{Enforcement Process} & \href{https://cdn.openai.com/papers/gpt-4-system-card.pdf}{Y} & \href{https://github.com/stanford-crfm/fmti/blob/main/scoring/Google%202023%20FMTI%20Scores.pdf}{N} & \href{https://console.anthropic.com/legal/aup}{Y} & \href{https://github.com/stanford-crfm/fmti/blob/main/scoring/Inflection%202023%20FMTI%20Scores.pdf}{N} & \href{https://github.com/stanford-crfm/fmti/blob/main/scoring/Meta%202023%20FMTI%20Scores.pdf}{N} & \href{https://docs.midjourney.com/docs/terms-of-service}Y \\
\textbf{Enforcement Justification} & \href{https://github.com/stanford-crfm/fmti/blob/main/scoring/OpenAI%202023%20FMTI%20Scores.pdf}{N} & \href{https://ai.google.dev/docs/safety_setting_gemini}{Y} & \href{https://github.com/stanford-crfm/fmti/blob/main/scoring/Anthropic%202023%20FMTI%20Scores.pdf}{N} & \href{https://heypisupport.zendesk.com/hc/en-us/articles/17791183959437-Understanding-Account-Suspension-Why-was-my-account-suspended-}{Y} & \href{https://github.com/stanford-crfm/fmti/blob/main/scoring/Meta%202023%20FMTI%20Scores.pdf}{N} & N \\
\textbf{Enforcement Appeal} & \href{https://github.com/stanford-crfm/fmti/blob/main/scoring/OpenAI%202023%20FMTI%20Scores.pdf}{Y} & \href{https://github.com/stanford-crfm/fmti/blob/main/scoring/Google%202023%20FMTI%20Scores.pdf}{N} & \href{https://github.com/stanford-crfm/fmti/blob/main/scoring/Anthropic%202023%20FMTI%20Scores.pdf}{N} & \href{https://web.archive.org/web/20230914081031/https://docs.google.com/forms/d/e/1FAIpQLScv5_-e6HjkvnqRBrpx8OG65PSAkX9XLXVMnE5eTpOdZQxF3Q/viewform}{Y} & \href{https://github.com/stanford-crfm/fmti/blob/main/scoring/Meta%202023%20FMTI%20Scores.pdf}{N} & Y \\
\bottomrule
\end{tabular}
\end{adjustbox}
% \captionsetup{justification=centering}
\caption{\TODO{update caption to reflect its just a copy with hyperlinks} We compile the policies, bounties, and types of access to each platform, beginning with six major players: OpenAI, Google, Anthropic, Meta, Inflection, and Midjourney. Each prescribes a prohibited set of uses, required by their terms of service, and all of these are enforced with moderation systems in the APIs and playgrounds, though only OpenAI and Anthropic openly disclose this. For instance, in GPT-4’s System Card OpenAI acknowledges using “a mix of reviewers and automated systems to identify and enforce against misuse”, and that policy-violating content will trigger warnings, suspensions and bans. OpenAI, Google, and Meta have bug bounties, but they are limited to traditional cybersecurity issues, excluding safety research. “Discloses Enforcement of Usage Policy” indicates whether the platform discloses its usage policy’s enforcement mechanisms. “Discloses Enforcement Justification” indicates whether a warning or suspension is accompanied by a justification to the user. “Enforcement Appeal Mechanism” indicates whether the user is given some way to appeal enforcement measures. The values for these are taken from indicators 75-77 of the Foundation Model Transparency Index. Taken together, inconsistent and poorly documented access and enforcement policies reduce the prevalence of red teaming efforts for generative AI systems.
\TODO{(* == Safe Harbor is "solely at their discretion")}
\TODO{Modify caption for Position paper. Mention OpenAI updated to protect "academic model safety" since reading an early draft of our piece.}
}
\label{tab:policies-hyperlinks}
\end{table*}
